A combinatorial DGA for Legendrian knots from generating families

For a Legendrian knot L in R^3 with a chosen Morse complex sequence (MCS) we construct a differential graded algebra (DGA) whose differential counts "chord paths" in the front projection of L. The definition of the DGA is motivated by considering Morse-theoretic data from generating families. In particular, when the MCS arises from a generating family we give a geometric interpretation of our chord paths as certain broken gradient trajectories which we call "gradient staircases". Given two equivalent MCS's we prove the corresponding linearized complexes of the DGA are isomorphic. If the MCS has a standard form, then we show that our DGA agrees with the Chekanov-Eliashberg DGA after changing coordinates by an augmentation.

==> Sections/BackgroundLagrAlgebra.tex <==
% ********************
\section{Background}
\mylabel{ch:Background}

A \emph{Legendrian knot} $\sLeg$ is a smooth knot in $\rr^3$ whose tangent space sits in the 2-plane distribution determined by the contact structure $\xi_{\text{std}} = \ker(dz-ydx)$. The projection of $\sLeg$ to the $xz$-plane is called the \emph{front projection} and the projection to the $xy$-plane is called the \emph{Lagrangian projection}. We will denote both projections by $\sLeg$ and, when necessary, provide context to prevent ambiguities. 

A Legendrian knot may be isotoped slightly to ensure the singularities in the front projection are transverse crossings and semicubical cusps. We say a front projection is in \emph{plat position} if the left cusps have the same $x$-coordinate, the right cusps have the same $x$-coordinate, and no two crossings have the same $x$-coordinate. A front projection $\sfront$ is \emph{nearly plat} if it is the result of perturbing a front projection in plat position slightly so that the cusps have distinct $x$-coordinates. Every Legendrian knot class admits a plat and, hence, a nearly plat representative and all Legendrian knots in this article are assumed to be nearly plat.  

The resolution algorithm defined by Ng in \cite{Ng2003} relates front and Lagrangian projections and, hence, provides an important bridge between invariants defined from these projections. The algorithm isotopes a front projection $\sfront$ to a front projection $\sfront'$ so that the Lagrangian projection of $L'$ is topologically similar to $\sfront$. Ng's resolution algorithm is an inductive process beginning to the left of $\sfront$ and proceeding to the right. Figure~\ref{f:Ng-resolution} describes the isotopy on $\sfront$ near crossings and cusps and the result of this isotopy in the Lagrangian projection. A \emph{strand} is a smooth path in $\sfront$ from a left cusp to a right cusp. The front $\sfront'$ is formed by stretching $\sfront$ in the $x$ direction and modifying the slopes of the strands of $\sfront$. The strands of $\sfront'$ have constant, decreasing slopes from top to bottom except near crossings and right cusps where the slopes of two consecutive strands are exchanged. Any front projection with strands arranged in this manner is said to be in \emph{Ng form}. By the Legendrian condition $y = \frac{dz}{dx}$, strands with constant slope correspond to strands with slope 0 in the resulting Lagrangian projection. The exchanging of two slopes results in a crossing in the resulting Lagrangian projection; see Figure~\ref{f:Ng-resolution}. Ng proves in \cite{Ng2003} that $\sfront$ and $\sfront'$ are front projections of Legendrian isotopic knots. 

\begin{figure}[t]
\centering
\includegraphics[scale=.5]{./images/Ng-resolution}
\caption[Stretching a left cusp.]{The resolution algorithm near a crossing, left cusp, and right cusp. From top to bottom, the three rows show the original front projection, stretched front projection and resulting Lagrangian projection.}
\label{f:Ng-resolution}
\end{figure}

Up to planar isotopy, the relationship between $\sfront$ and the resulting Lagrangian projection is as follows. Given a Legendrian knot with front projection $\sfront$, we form the \emph{Ng resolution}, denoted $\sNgres$, by smoothing the left cusps as in\footnote{This figure is essentially contained in the previous one.  Could we possibly do without it?} Figure~\ref{f:Ng-procedure}~(a), smoothing and twisting the right cusps as in Figure~\ref{f:Ng-procedure}~(b), and resolving the double points as in Figure~\ref{f:Ng-procedure}~(c).

\begin{figure}[t]
\labellist
\small\hair 2pt
\pinlabel {(a)} [tl] at 30 12
\pinlabel {(b)} [tl] at 113 12
\pinlabel {(c)} [tl] at 210 12
\endlabellist
\centering
\includegraphics[scale=.7]{./images/Ng-procedure}
\caption{Resolving the cusps and crossings of a front projection to form the Ng resolution.}
\label{f:Ng-procedure}
\end{figure}

The Legendrian contact homology of Eliashberg and Hofer \cite{Eliashberg2000} provides a differential graded algebra that has given rise to many Legendrian invariants. In \cite{Chekanov2002a}, Chekanov formulates the differential graded algebra combinatorially and extracts a Legendrian invariant capable of distinguishing Legendrian knot classes not distinguished by the classical invariants. The resulting differential graded algebra is known as the \emph{Chekanov-Eliashberg differential graded algebra}, abbreviated CE-DGA and denoted $(\salg(\sLeg), \df)$. We refer the reader to any of \cite{Chekanov2002a,Chekanov2002,Etnyre2002,Sabloff2005} for a more complete introduction to the CE-DGA. 

The algebra $\salg(\sLeg)$ is the unital tensor algebra of the $\zz_2$ vector space $A(L)$ freely generated by labels $Q = \{q_1, \hdots, q_n \}$ assigned to the crossings of the Lagrangian projection $\sLagr$. 

\begin{remark}
In this article, we will work with Legendrian knots admitting generating families, so we may make the assumption that the classical invariant known as the rotation number is $0$.  Then,    $(\salg(\sLeg), \df)$
has a $\zz$-grading which, as a Lagrangian projection is assumed to correspond to the resolution of a front projection, may be defined in terms of a Maslov potential on the front projection of $\sLeg$. 
\end{remark}

\begin{figure}[t]
\labellist
\small\hair 2pt
\pinlabel {(a)} [tl] at 46 4
\pinlabel {(b)} [tl] at 160 4
\pinlabel {$i$} [tl] at 5 11
\pinlabel {$i+1$} [br] at 13 27
\pinlabel {$i$} [tl] at 102 11
\pinlabel {$i+1$} [bl] at 102 27
\pinlabel {$+$} [tl] at 147 24
\pinlabel {$+$} [tl] at 184 24
\pinlabel {$-$} [tl] at 164 35
\pinlabel {$-$} [tl] at 164 13
\endlabellist
\centering
\includegraphics[scale=1]{./images/maslov}
\caption[]{(a) The Maslov relation near cusps. (b) Reeb signs near a crossing.}
\label{f:Maslov}
\end{figure}

\begin{definition}
	\mylabel{defn:Maslov}	A \emph{Maslov potential} on $\sfront$ is a map $\sMaslov$ from the front projection of $\sLeg$ to $\Z$ which is constant except at cusps where it satisfies the relation shown in Figure~\ref{f:Maslov}.
\end{definition}

The grading on $(\salg(\sLeg), \df)$ is defined on generators and then extended additively to  $\salg(\sLeg)$.
If $q \in Q$ corresponds to a resolved right cusp, then $|q|=1$. If $q$ corresponds to a resolved crossing, then $|q| = \sMaslov(T) - \sMaslov(B)$ where $T$ and $B$ are the strands crossing at $q$ and $T$ has smaller slope. 

The differential $\df$ counts certain immersed disks in the $xy$-plane with convex corners at crossings. We follow the definition of $\df$ given in \cite{Chekanov2002a} and \cite{Etnyre2002}. Decorate the quadrants of the crossings of $\sLagr$ with $+$ and $-$ signs as in Figure~\ref{f:Maslov}~(b). Let $D$ be the unit disk in $\rr^2$ and let $\xxc = \{ x_0, \hdots, x_n \}$ be a set of distinct points along $\df D$ in counter-clockwise order. A \emph{convex immersed polygon} is a continuous map $f : D \to \rr^2$ so that:
	\begin{enumerate}
		\item $f$ is an orientation-preserving immersion on the interior of $D$;
		\item The restriction of $f$ to $\df D \setminus \xxc$ is an immersion whose image lies in the Lagrangian projection of $\sLagr$; and
		\item The image of each $x_i \in \xxc$ under $f$ is a crossing of $\sLagr$, and the image of a neighborhood of $x_i$ covers a convex corner at the crossing. Call a corner of an immersed polygon \emph{positive} if it covers a $+$ sign and \emph{negative} otherwise.
	\end{enumerate}
We define $\widetilde{\Delta} (q_i; q_{j_1}, \hdots, q_{j_k})$ to be the set of convex immersed polygons with a positive corner at $q_i$ and negative corners at $q_{j_1}, \hdots, q_{j_k}$. The negative corners are ordered by the counter-clockwise order of the marked points along $\df D$. Let $\Delta (q_i; q_{j_1}, \hdots, q_{j_k})$ be $\widetilde{\Delta} (q_i; q_{j_1}, \hdots, q_{j_k})$ modulo smooth reparameterization.

\begin{definition}
	\mylabel{defn:DGA-boundary}
	The differential $\df$ on the algebra $\aac(\sLagr)$ is defined on a generator $q_i \in Q$ by the formula:
	\begin{equation}
		\mylabel{eq:DGA-diff}
		\df q_i = \sum_{\Delta (q_i; q_{j_1}, \hdots, q_{j_k})} \# (\Delta (q_i; q_{j_1}, \hdots, q_{j_k})) q_{j_1} \hdots q_{j_k}
	\end{equation}
	\noindent where $\# (\Delta (\hdots))$ is the mod 2 count of the elements in $\Delta (\hdots)$. We extend $\df$ to all of $\aac(\sLagr)$ by linearity and the Leibniz rule. 
\end{definition}

\begin{theorem}[\cite{Chekanov2002a}]
	\mylabel{thm:CE-DGA-diff}
	The differential $\df$ satisfies:
	\begin{enumerate}
		\item The sum in equation~(\ref{eq:DGA-diff}) is finite;
		\item $| \df q | = |q| - 1 $ modulo $2 r(K)$; and 
		\item $\df \circ \df = 0$.
	\end{enumerate}
	The homology of the CE-DGA $(\aac(\sLagr), \df)$ is a Legendrian isotopy invariant, as is its stable-tame isomorphism class.
\end{theorem}

In \cite{Chekanov2002a} and \cite{Chekanov2002}, Chekanov considers a type of algebra homomorphism on $(\aac(\sLagr), \df)$, called an augmentation, which allows us to extract a finite dimensional linear chain complex from the infinite dimensional DGA $(\aac(\sLagr), \df)$. These maps, along with the resulting linear homology groups, have provided easily computable Legendrian knot invariants. An \emph{augmentation} is an algebra map $\saug : (\aac(\sLagr), \df) \to \zz_2$ satisfying $\saug(1) = 1$, $\saug \circ \df = 0$, and if $\saug (q_i) = 1$ then $ |q_i| = 0 $. We let $Aug(\sLagr)$ denote the set of augmentations of $(\aac(\sLagr), \df)$. Given $\saug \in Aug(\sLagr)$ we define the algebra homomorphism $\phi^{\saug} : \aac(\sLagr) \to \aac(\sLagr)$ to be the extension of the map on generators given by $\phi^{\saug}(q) = q + \saug(q)$. This allows us to consider an alternate differential on $\aac(\sLagr)$ defined by $\df^{\saug}= \phi^{\saug} \df (\phi^{\saug})^{-1}$.

As a vector space, $\aac(\sLagr)$ decomposes as $\aac(\sLagr)= \bigoplus_{n=0}^{\infty} A(L)^{\otimes n}$ where $A(L)^{\otimes 0}=\zz_2$ and $A(L)^{\otimes n}$ is spanned by the monomials of length $n$ in the generators from $Q$. The differential $\df$ decomposes as $\df = \sum_{n=0}^{\infty} \df_n$ where $\df_n q$ is the sum of monomials of length $n$ in $\df q$. The differential $\df^{\saug}$ has the comparative advantage that $\df^{\saug}_0 = 0$. Thus, $(\df_1^{\saug})^2=0$ and $(A(L), \df_1^{\saug})$ is a finite dimensional chain complex  with homology groups $LCH_{*}^{\saug}(\sLagr)$ called the \emph{linearized contact homology of $\saug$}. The set of homology groups $\{LCH_{*}^{\saug}(\sLagr)\}_{\saug \in Aug(\sLagr)}$ is a Legendrian knot invariant.

%%-----------------------------------------------------------
\subsection{Generating Families}
\mylabel{sec:Gen-fams}
%%-----------------------------------------------------------
Consider a function $F : \rr \times \rr^N \to \rr$.  We use coordinates $(x, e), x\in \rr$ and $e\in \rr^N$ for the domain which shall be viewed as a trivial vector bundle over $\rr$.  
Denote by $S_F$ the {\it fiber critical set}
\[
S_F = \left \{ (x,e) \, \left | \, \frac{\partial F}{\partial e}(x,e) = 0 \right \} \right..
\]
We will assume the matrix $\displaystyle \left [ \frac{\partial^2 F}{\partial x \partial e}(x,e) \, \frac{\partial^2 F}{\partial e^2}(x,e) \right ]$ has full rank at all $(x,e) \in S_F$, thus $S_F$ is a $1$-dimensional submanifold of $\rr \times \rr^N$.  Then the map
\[
i_F : S_F \to \rr^3, \quad i_F(x,e) = \left (x, \frac{\partial F}{\partial x}(x,e), F(x, e) \right )
\]
gives a Legendrian immersion.  If $L \subset \rr^3$ is a Legendrian knot or link with $i_F(S_F)= L$ we say that $F$ is a {\it generating family} for $L$. Figure~\ref{f:gen-fam-example} gives a generating family for a Legendrian unknot. We will require generating families to  be {\it linear at infinity}.  That is, $F$ should be equal to some nonzero linear function, $F(x,e) = l(e)$, outside of a compact subset $K \subset \rr \times \rr^N$. 

\begin{figure}[t]
\labellist
\small\hair 2pt
\pinlabel {$x$} [tl] at 958 217
\pinlabel {$z$} [tl] at 115 491
\pinlabel {$x_4$} [tl] at 430 238
\pinlabel {$F(x_4, \cdot)$} [tl] at 490 190
\endlabellist
\centering
\includegraphics[scale=.34]{./images/gen-fam-example}
\caption[A generating family for a Legendrian unknot.]{A linear at infinity generating family $F : \rr \times \rr \to \rr$ for a Legendrian unknot $L$. The graph of $F(x, \cdot): \rr \to \rr$ is given for several values of $x$. The four intersection points of $L \cap (\{x_4\} \times \rr)$ correspond to the four critical points of $F(x_4, \cdot)$.}
\label{f:gen-fam-example}
\end{figure} 

\begin{remark}  Not all Legendrian links $L \subset \rr^3$ admit generating families.  In fact, $L$ admits a linear at infinity generating family if and only if $L$ has a graded normal ruling.  These conditions are in turn equivalent to the existence of a graded augmentation of the Chekanov-Eliashberg DGA. See \cite{Chekanov2005}, \cite{Fuchs2003}, \cite{Fuchs2004}, \cite{Fuchs2008}, \cite{Ng2006}, and \cite{Sabloff2005} for details on these results.
\end{remark}


==> Sections/Chord-Path.tex <==
% ********************
\section{Associating a DGA to an MCS}
\mylabel{ch:DGA-to-MCS}

Content: Associate to an MCS a graded algebra and a map $\df$ by counting certain chord paths. 

%%-----------------------------------------------------------
\subsection{$\df^2 = 0$} 
\mylabel{sec:d2=0}
%%-----------------------------------------------------------

Content: Prove $\df^2 = 0$.

%%-----------------------------------------------------------
\subsection{One-dimensional moduli spaces of chord trees} 
\mylabel{sec:Moduli-spaces}
%%-----------------------------------------------------------

Content: Define the trees representing the one-dimensional moduli spaces of gradient trees.

%%-----------------------------------------------------------
\subsection{Equivalent MCSs induce isomorphic linearized DGAs} 
\mylabel{sec:Linear-inv}
%%-----------------------------------------------------------

Content: Use the one-dimensional moduli space to prove that equivalent MCSs induce isomorphic linearized DGAs.



==> Sections/Figures.tex <==
% ********************
\section{Figures}
\mylabel{ch:figures}

This is just a storage space for figures I have made until we find a place for them in the paper.


\begin{figure}[t]
\centering
\includegraphics[scale=.4]{./images/mcs-example}
\caption[An MCS for a Legendrian unknot.]{An MCS for a Legendrian unknot.}
\label{f:mcs-example}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=.5]{./images/mcs-trefoil-example}
\caption[An MCS for a Legendrian trefoil.]{An MCS for a Legendrian trefoil.}
\label{f:mcs-example}
\end{figure}




==> Sections/Preamble.tex <==
% This is the preamble of the document where Theorem-type environments are defined. Common shortcuts and document-specific notation are also defined here.
% Michael Brad Henry

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\makeatletter
\newtheorem*{rep@corollary}{\rep@title}
\newcommand{\newrepcorollary}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@corollary}}%
 {\end{rep@corollary}}}
\makeatother

% Theorems and such
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newreptheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newrepcorollary{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{property}{Property}
\newtheorem{step}{Step}
\newtheorem*{condition}{Condition}
\newtheorem{question}{Question}
\newtheorem{remark}[theorem]{Remark}

\theoremstyle{remark}
\newtheorem*{example}{Example}
\newtheorem*{note}{Note}


% Shortcut to ``blackboard bold'' and script letters
\newcommand{\cc}{\ensuremath{\mathbb{C}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\rr}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\zz}{\ensuremath{\mathbb{Z}}}
\newcommand{\qq}{\ensuremath{\mathbb{Q}}}
\newcommand{\pp}{\ensuremath{\mathbb{P}}}
\newcommand{\nn}{\ensuremath{\mathbb{N}}}
\newcommand{\aac}{\ensuremath{\mathcal{A}}}
\newcommand{\bbc}{\ensuremath{\mathcal{B}}}
\newcommand{\rrc}{\ensuremath{\mathcal{R}}}
\newcommand{\wwc}{\ensuremath{\mathcal{W}}}
\newcommand{\vvc}{\ensuremath{\mathcal{V}}}
\newcommand{\ttc}{\ensuremath{\mathcal{T}}}
\newcommand{\ssc}{\ensuremath{\mathcal{S}}}
\newcommand{\llc}{\ensuremath{\mathcal{L}}}
\newcommand{\kkc}{\ensuremath{\mathcal{K}}}
\newcommand{\nnc}{\ensuremath{\mathcal{N}}}
\newcommand{\xxc}{\ensuremath{\mathcal{X}}}
\newcommand{\mmc}{\ensuremath{\mathcal{M}}}


%Definitions of document-specific notation
\newcommand{\sAugL}{\ensuremath{Aug(\mathcal{A}(L))}}
\newcommand{\df}{\ensuremath{\partial}}
\newcommand{\sMCS}{\ensuremath{\mathcal{C}}}
\newcommand{\sbMCS}{\ensuremath{[\mathcal{C}]}}
\newcommand{\sMCSeq}{\ensuremath{\sim}}
\newcommand{\sFMCS}{\ensuremath{MCS(\sfront)}}
\newcommand{\sSMCS}{\ensuremath{MCS_S(\sfront)}}
\newcommand{\sAMCS}{\ensuremath{MCS_A(\sfront)}}
\newcommand{\sFMCSeq}{\ensuremath{\widehat{MCS}(\sfront)}}
\newcommand{\salg}{\ensuremath{\mathcal{A}}}
\newcommand{\sHSM}{\ensuremath{\mathcal{H}}} %Matrix of a Handleslide Move
\newcommand{\sdmatrix}{\ensuremath{\mathcal{D}}} %Matrix of the differential of an ordered chain complex
\newcommand{\sLeg}{\ensuremath{L}} %A Legendrian knot. We also use $L$ to refer to the Legendrian isotopy class.
\newcommand{\sLagr}{\ensuremath{L}} %The Lagrangian projection.
\newcommand{\sfront}{\ensuremath{L}} %The front projection of a Legendrian knot $K$.
\newcommand{\sNgres}{\ensuremath{L_N}} %The Ng resolution of a front projection.
\newcommand{\sMaslov}{\ensuremath{\mu}} %A Maslov potential.
\newcommand{\sgenfam}{\ensuremath{F}} %A generating family for a Legendrian front projection.
\newcommand{\saug}{\ensuremath{\epsilon}} %An augmentation.


%Extra and possibly unnecessary code of unknown origin. I am hesistant to remove it until I am sure it is unneeded.

% Adrian's magic label command
\newcommand{\mylabel}[1]{\label{#1}
%Comment this part out to remove the label boxes
%\fbox{\upshape \tiny {#1}}
}

\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
